Toward Multiple Specialty Learners for Explaining GNNs via Online Knowledge Distillation

Graph Neural Networks (GNNs) have become increasingly ubiquitous in numerous applications and systems, necessitating explanations of their predictions, especially when making critical decisions. However, explaining GNNs is challenging due to the complexity of graph data and model execution. Despite additional computational costs, post-hoc explanation approaches have been widely adopted due to the generality of their architectures. Intrinsically interpretable models provide instant explanations but are usually model-specific, which can only explain particular GNNs. Therefore, we propose a novel GNN explanation framework named SCALE, which is general and fast for explaining predictions. SCALE trains multiple specialty learners to explain GNNs since constructing one powerful explainer to examine attributions of interactions in input graphs is complicated. In training, a black-box GNN model guides learners based on an online knowledge distillation paradigm. In the explanation phase, explanations of predictions are provided by multiple explainers corresponding to trained learners. Specifically, edge masking and random walk with restart procedures are executed to provide structural explanations for graph-level and node-level predictions, respectively. A feature attribution module provides overall summaries and instance-level feature contributions. We compare SCALE with state-of-the-art baselines via quantitative and qualitative experiments to prove its explanation correctness and execution performance. We also conduct a series of ablation studies to understand the strengths and weaknesses of the proposed framework.

==> egcn.tex <==
\begin{picture}(70,30)
    \put(23,25){\textbf{\small EGCN}}
    \end{picture}
    \subfloat{%
        \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/egcn_ba_shape_410.pdf}
        \label{fig:ba_shape}
     }
     \hfil
     \subfloat{%
        \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/egcn_ba_community_410.pdf}
        \label{fig:ba_community_510}
     }
     \hfil
    \subfloat{%
        \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/egcn_tree_cycle_511.pdf}
        \label{fig:tree_cycle_517}
     }
     \hfil
    \subfloat{%
        \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/egcn_tree_grid_511.pdf}
        \label{fig:masktempl}
     }
     \hfil
     \subfloat{%
        \includegraphics[width=0.12\linewidth]{figures/graphs/blank.pdf}
        \label{fig:ba_shape}
     }
     \hfil
     \subfloat{%
        \includegraphics[width=0.12\linewidth]{figures/graphs/blank.pdf}
        \label{fig:ba_shape}
     }
     \hfil

==> trash.tex <==
% Furthermore, post-hoc training models usually encounter the overfitting problem as the training data for them are usually small or only a subset of the original dataset. Even worse, they are trained with ground-truth labels resulting in discrimination between them and the base model
% Essential subgraph detection is the main focus of recent explanation methods for GNNs, wherein edges contributing more to a prediction are given higher probabilities. 
% However, most current approaches require an additional training process to learn edge importance. 
% Besides, existing methods usually assumed that interpretations outputted by post-hoc training techniques reflect the original model behaviors. This assumption can only be obtained when both the base model and the surrogate model have high accuracy scores. 



% Besides, if we set the preference vector in PageRank to a specific set of nodes, we obtain a hierarchical structure of influential nodes to this set, which can be used for explaining predictions of node classification or link prediction. This approach requires GNNs to have a matrix that represents transition probabilities between nodes, denoted as $\hat{\mathcal{A}}$. Based on online knowledge distillation, this matrix is constructed on-the-fly during model training.
% Link analysis algorithms like PageRank are alternative methods to examine the contributions of the network structure in predictions.

% Moreover, graphs are only loaded one time into GPUs, thus avoiding GPU memory redundancy, unlike \cite{ying2019gnnexplainer,luo2020parameterized}.

% When $\lambda \leq 1$, the self-explainable GNN model masked out all edges of graphs in one class and can only highlight important edges of graphs in the other class, thus resulting in inferior explanation results for the BA-2motif dataset


\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        Methods     & \thead{Re-\\train} & \thead{Expl.\\Speed} & \thead{Expl.\\Quality} & Approach\\
        \hline
       GNNExplainer \cite{ying2019gnnexplainer} & Y & Slow & High & Agnostic\\
       PGExplainer \cite{luo2020parameterized}  & Y & Slow & High & Agnostic\\
       \hline
       GCN-MLP      & N & Fast & Medium & Specific\\
       GAT \cite{velickovic2017graph}   & N & Fast & Medium & Specific\\ 
       SEGNN \cite{dai2021towards}       & N & Fast & Low & Specific\\
       EGNN \cite{li2022egnn} & N & Slow & Low & Specific\\
       \hline
       PGX          & N & Fast & High & Hybrid\\
       \hline
    \end{tabular}
    \vspace{0.2cm}
    \caption{A Summary of Method Performances. PGX outperforms post-hoc methods in all comparisons, while it is comparable to self-explainable methods in execution speed.}
    \label{tab:all_baselines}
\end{table}


% \begin{picture}(70,30)
    % \put(0,28){\textbf{\small GNNExplainer}}
    % \end{picture}
    % \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/gnn_ba_shapes_410.pdf}
    %     % \label{fig:ba_shape}
    %  }
    %  \hfil
    %  \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/gnn_ba_community_410.pdf}
    %     % \label{fig:ba_community_510}
    %  }
    %  \hfil
    % \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/gnn_tree_cycle_517.pdf}
    %     % \label{fig:tree_cycle_517}
    %  }
    %  \hfil
    % \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/gnn_treegrid_511.pdf}
        
    %  }
    %  \hfil
    %  \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_ba2motif_5.pdf}
    %  }
    %  \hfil
    %  \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_mutag_257.pdf}
    %  }
    %  \hfil
    % \vspace{-0.2cm}
    
    % \begin{picture}(70,30)
    % \put(0,28){\textbf{\small PGExplainer}}
    % \end{picture}
    % \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_ba_shapes_410.pdf}
    %     % \label{fig:ba_shape}
    %  }
    %  \hfil
    %  \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_ba_community_410.pdf}
    %     % \label{fig:ba_community_510}
    %  }
    %  \hfil
    % \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_tree_cycle_517.pdf}
    %     % \label{fig:tree_cycle_517}
    %  }
    %  \hfil
    % \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_treegrid_511.pdf}
    %  }
    %  \hfil
    %  \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_ba2motif_5.pdf}
    %  }
    %  \hfil
    %  \subfloat{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/pg_mutag_257.pdf}
    %  }
    %  \hfil
    % \vspace{-0.2cm}
    % \begin{picture}(70,30)
    % \put(35,28){\textbf{\small PGX}}
    % \end{picture}
    % \setcounter{subfigure}{0}
    % % \hspace{-0.239cm}
    % \subfloat[BA Shapes]{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/ba_shape_510_2.pdf}
    %     \label{fig:ba_shape}
    %  }
    %  \hfil
    %  \hspace{-0.239cm}
    %  \subfloat[BA Community]{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/ba_community_510.pdf}
    %     \label{fig:ba_community_510}
    %  }
    %  \hfil
    % \subfloat[Tree Cycle]{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/tree_cycle_517_l3.pdf}
    %     \label{fig:tree_cycle}
    %  }
    %  \hfil
    % \subfloat[Tree Grid]{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/tree_grid_511.pdf}
    %     \label{fig:tree_grid}
    %  }
    %  \hfil
    %  \subfloat[BA-2motifs]{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/ba2motif_1.pdf}
    %     \label{fig:ba2motif}
    %  }
    %  \hfil
    %  \subfloat[Mutag]{%
    %     \includegraphics[clip,trim=2.5cm 2.5cm 2.0cm 2.4cm,width=0.12\linewidth]{figures/graphs/mutag_257.pdf}
    %     \label{fig:mutag}
    %  }
    %  \hfil
    
% Next, an explainable GNN model is trained to capture edge importance. Referred to \cite{luo2020parameterized}, SCALE initializes this mask by passing concatenated vectors of source and target node embeddings taken from the black-box GNN to a multi-level perceptron (MLP) network. Moreover, a feature attribution module includes an MLP model, which tries to imitate the black-box GNN predictions. This model is later used for generating feature attributions at different levels.
